A new Local Radon Descriptor for Content-Based Image Search

Content-based image retrieval (CBIR) is an essential part of computer vision research, especially in medical expert systems. Having a discriminative image descriptor with the least number of parameters for tuning is desirable in CBIR systems. In this paper, we introduce a new simple descriptor based on the histogram of local Radon projections. We also propose a very fast convolution-based local Radon estimator to overcome the slow process of Radon projections. We performed our experiments using pathology images (KimiaPath24) and lung CT patches and test our proposed solution for medical image processing. We achieved superior results compared with other histogram-based descriptors such as LBP and HoG as well as some pre-trained CNNs.

==> A new Local Radon-based Descriptor for Content-Based Image Search/table.tex <==
\begin{table}[!h!t] 
	\caption{The best results for all datasets and descriptors when city block ($L_1$), Euclidean ($L_2$), Chi-squared ($\chi^2$) and cosine ($\cos$) distances are used for direct similarity measurements. For LBP and HOG, the best results were achieved for each dataset via exhaustive parameter search.}
	\begin{center}
		\begin{tabular}{lcll}
			\toprule
			\multicolumn{3}{l}{\cellcolor{gray!25} \textbf{CT Emphysema Dataset}}\\
			\multicolumn{3}{l}{\cellcolor{gray!25} }\\
			Method & $A_\textrm{CT}$ & $|\mathbf{h}|$ \\	
			\toprule
			\vspace{0.05in}
			LRP(Our method)$_\textrm{MinMax}$ 	 	  	& 82.14\% & 2048	&   \\ \vspace{0.05in}	
			LRP(Our method)$_\textrm{median}$ 	 	  	& 81.32\% & 4096	&   \\ \vspace{0.05in}	
			ELP \cite{tizhoosh2018representing}$_\textrm{median}$ 	 	  	& 80.95\% & 256	&   \\ \vspace{0.05in}
			LBP$^{uri}_{(12,3), \chi^2}$		 	 & 80.36\%	& 18 	&  	\\ \vspace{0.05in}
			VGG-Deep$_{L_2}$\cite{kumar2018deep}			  	& 	69.64\% & 4096	&  \\ 
			\vspace{0.05in}	
			HOG$_{L_2}$			 	  	& 65.47\%	& 1215	&  	\\ 
			\bottomrule
			\multicolumn{3}{l}{\cellcolor{gray!25} \textbf{Kimia Path24 Dataset}}\\ 
			\multicolumn{3}{l}{\cellcolor{gray!25}}\\ 
			Method & $ \{\eta_p,\eta_W\}$ & $|\mathbf{h}|$ &   \\	
			\toprule
			\vspace{0.05in}
			LRP(Our method)$_\textrm{median}$  		  	& \{75.38\%, 72.02\%\} & 4096	 \\ \vspace{0.05in}
			LRP(Our method)$_\textrm{MinMax}$  		  	& \{74.12\%, 73.43\%\} & 2048	 \\ \vspace{0.05in}
			ELP \cite{tizhoosh2018representing}$_\textrm{median}$ 	 	  	& \{71.16\%, 68.05\%\} & 1024	&   \\
			VGG-Deep$_{\cos}$\cite{kumar2018deep}			  	& \{70.11\%, 68.13\%\}	 & 4096	&  	\\ \vspace{0.05in}	
			LBP$^u_{(24,2), L_1}$		 	 & \{65.55\%, 62.56\%\}	 & 555	&  	\\ \vspace{0.05in}	
			HOG$_{L_1}$			 	  	& \{17.58\%, 16.76\%\}	 & 648	&  	\\ 
			
		\end{tabular}
	\end{center}
	\label{tab:subimages}
\end{table}%	
